Controller Synthesis for Omega-Regular and Steady-State Specifications

Given a Markov decision process (MDP) and a linear-time ($\omega$-regular or LTL) specification, the controller synthesis problem aims to compute the optimal policy that satisfies the specification. More recently, problems that reason over the asymptotic behavior of systems have been proposed through the lens of steady-state planning. This entails finding a control policy for an MDP such that the Markov chain induced by the solution policy satisfies a given set of constraints on its steady-state distribution. This paper studies a generalization of the controller synthesis problem for a linear-time specification under steady-state constraints on the asymptotic behavior. We present an algorithm to find a deterministic policy satisfying $\omega$-regular and steady-state constraints by characterizing the solutions as an integer linear program, and experimentally evaluate our approach.

==> __latexindent_temp.tex <==
\begin{equation}
	\nonumber
	\begin{aligned}
	\theta & \triangleq \textbf{true } \mid \theta_1 \wedge \theta_2 \mid \neg \theta \mid \phi   \\
	\phi & \triangleq  p \mid \textbf{ SS}_{[l, u]} (p) \mid \phi_1 \wedge \phi_2 \mid \neg \phi \mid \textbf{X} \phi \mid \phi_1 \textbf{U} \phi_2.
	\end{aligned}
	\end{equation}

==> ccp.tex <==

%even  that all BSCCs of the product MC induced by $\pi$ contain the same set of states in $S$. That is,  the contrapositive. Assume that, for a given policy $\pi$, $\mathcal{M}_\pi = (S_\pi, T_\pi)$ is not recurrent, where $S_\pi = \{s \in S : \mathcal{I}_s = 1\}$. We will demonstrate that the values of $\pi$ which induce this Markov chain violate constraints in the program. It follows that there exists some node $s^* \in S_\pi$ such that there is either no path from $S_\beta$ to $s^*$ in $\mathcal{M}_\pi$ or from $s^*$ to $S_\beta$ in $\mathcal{M}^\text{rev}_\pi$ (This is $\mathcal{M}_\pi$ with the edges reversed). We will focus on the former case since a similar argument applies to both cases. 
		
		%For any possible path from $S_\beta$ to $s^*$ in the underlying LMDP $\mathcal{M}$, there exists some edge $(s, s') \in T^\text{rel}$ such that $T_\pi(s' | s) = 0$. From equation (\ref{equation:proof}) below, this implies that $f_{s,s'} = 0$ for all such edges. This, in turn, violates constraint $(vii)$ as it requires non-zero incoming flow into $s^*$ (recall that $\mathcal{I}_{s^*}$) and $s^*$ is disconnected from the originators of flow in $S_\beta$. By originator of flow, we mean that any state in $S_\beta$ can have higher outgoing flow than incoming flow as defined in constraint $(vii)$. Therefore, all incoming flow into any vertex must have a path from $S_\beta$.
		
		%\begin{equation}
		%\begin{aligned}
		%f_{sqs'q'} & \leq \sum_{a \in A(s)} T^\times ((s', q') | (s, q), a) \pi(a | s) \\ 
		%& = \sum_{a \in A(s)} \text{Pr}_\pi((s', q') a | (s, q)) = T^\times_\pi ((s', q') | (s, q))
		%\end{aligned}
		%\label{equation:proof}
		%\end{equation}
		
		%($\impliedby$) Since $\mathcal{M}_\pi$ is recurrent, there exists a path between every pair of nodes $(s_{\text{start}}, s_{\text{end}}) \in T^{\text{rel}}_\pi$, where $T^{\text{rel}}_\pi = \{(s, s') \in S \times S | s \neq s' \wedge T_\pi (s' | s) > 0\} \subseteq T^\text{rel}$ denotes the graph structure of $\mathcal{M}_\pi$. For every pair of adjacent nodes $(s, s')$ in such a path, we have $T_\pi (s' | s) > 0$. From equation (\ref{equation:proof}), we have that $f_{s, s'} \leq T_\pi (s' | s)$. We can thus assign non-zero values to all flow variables $f_{s, s'}$ whose corresponding transition probabilities $T_\pi (s' | s)$ are non-zero. This satisfies constraint $(v)$. Note that these values can be arbitrarily chosen so that constraint $(vii)$ holds. It follows from the recurrence of $\mathcal{M}_\pi$ that there is incoming flow into every $s \in S_\pi$, thereby satisfying constraint $(ix)$. Similar arguments with regards to the reverse graph of $\mathcal{M}_\pi$ can be made to establish the satisfiability of constraints $(vi)$, $(viii)$, and $(x)$. \qed
	%\end{proof}
	

	
	%\begin{corollary}
		%Given a DSSPS instance $\left< \mathcal{M} = (S, A, T, R, L), \Phi \right>$, the integer linear program (\ref{program2_2}) is feasible if and only if there exists a deterministic policy $\pi: S \times A \mapsto \{0, 1\}$ such that the induced Markov chain $\mathcal{M}_\pi = (S_\pi, T_\pi)$ is recurrent and satisfies the specifications in $\Phi$.
	%\end{corollary}

	%\begin{proof}
		%This follows directly from Theorems $1$ and $2$. \qed
		%It follows from Theorem $1$ that $\mathcal{M}_\pi$ is recurrent. From Theorem $2$, we know that the identity $\pi (a | s) = x_{sa} / \text{Pr}^\infty_\pi (s)$ holds. 
	%\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% TeX-PDF-mode: t
%%% End:

==> discussion.tex <==
Hi

==> finalLong.tex <==
%appendix goes here
\newpage
\section{Product LMDP Construction Example}
\label{fig:prod}
\begin{center}
\includegraphics[width=10cm]{combined.pdf}
\end{center}

Consider the figure shown above.
(a) LMDP $\mathcal{M} = (S, \beta, A, T, R = \emptyset, AP, L)$, where $S = \{s_0, \dots, s_6\}$, $\beta(s_4) = 1$, $A = \{a_0, \dots, a_3\}$, $AP = \{a, c\}$, and $L(s_0) = L(s_1) = L(s_2) = \{a\}, L(s_3) = \{c\}$. The transition function is deterministic and shown in the figure by the transitions $a_i:1$ between states $s, s'$ denoting that $T(s, a_i)(s') = 1$. The blue transitions define a policy $\pi$ which induces a unichain LMC $\mathcal{M}_\pi$ (The isolated component consisting of states $s_5$ and $s_6$ is ignored since it is unreachable). (b) The DRA $\mathcal{A} = (Q, q_0, \Sigma, \delta, F = \{(B_i, G_i)\}_i)$ is shown, where $Q = \{q_0, q_1, q_2\}$, $\Sigma = 2^{AP}$, $F = \{(\emptyset, \{q_2\})\}$ and $!, \&$ denote negation and conjunction. (c) Product LMDP $\mathcal{M} \times \mathcal{A}$, where red nodes represent states in the AMEC of $\mathcal{M} \times \mathcal{A}$. The blue transitions define the product LMC $(\mathcal{M} \times \mathcal{A})_\pi$ induced by the policy $\pi$. Note that this policy induces an LMC that has probability 1 of being trapped in the accepting MEC. Therefore, the probability of satisfying the $\omega$-regular property represented by $\mathcal{A}$ given that we start in state $s_0$ is 1.

% \begin{figure}[h!]
%     \centering
%     \label{fig:example}
% \end{figure}

\section{Example Illustrating SS+LTL Specifications}
\label{fig:ss+ltl}
\begin{center}
	\includegraphics[width=\columnwidth]{example2NewNew.PNG}
\end{center}
	(a) LMDP $\mathcal{M} = (S, \beta, A, T, R = \emptyset, AP, L)$, where $S = \{s_0, \dots, s_8\}$, $\beta(s_0) = 1$, $A = \{\leftarrow, \downarrow, \rightarrow, \uparrow\}$, $AP = \{home, danger, tool\}$, and $L(s_0) = \{home\}, L(s_1) = L(s_7) = \{danger\}, L(s_8) = \{tool\}$. the agent has a chance of slipping whenever it moves, causing a transition into one of three possible states. If the agent chooses to go right (left), there is an 80$\%$ chance that it will transition to the right (left), and the chance of transitioning to either of the states above or below it is 10$\%$ each. Similarly, if the agent chooses to go up (down), it will end up in the states above (below) it with 80$\%$ chance, and in the states to the right and left of it with probability 10$\%$ each. In the corners of the map, the agent may stay in place with 90$\%$ probability by choosing to move against the boundary of the map (e.g. $T(s_0, \leftarrow)(s_0) = 0.9$). (b) Given the SS+LTL specification $\theta = ((! danger \textbf{U} tool), \textbf{SS}_{[0.75, 1]} home)$, the corresponding LTL DRA $\mathcal{A} = (Q, q_0, \Sigma, \delta, F = \{(B_i, G_i)\}_i)$ is defined, where $Q = \{q_0, q_1, q_2\}$, $\Sigma = 2^{AP}$, $F = \{(\emptyset, \{q_1\})\}$, and the transition function is given by $\delta(q_0, \emptyset) = q_0, \delta(q_0, \{tool\}) = q_1, \delta(q_0, \{danger\}) = q_2, \delta(q_1, \cdot) = q_1, \delta(q_2, \cdot) = q_2$. The symbols $!, \&$ denote negation and conjunction. Note that the steady-state specification in $\theta$ is not used in defining $\mathcal{A}$. (c) Product LMC $(\mathcal{M} \times \mathcal{A})_\pi$ induced by the policy $\pi$ given by the black arrows in (a) for the product LMDP $\mathcal{M} \times \mathcal{A}$, where red nodes represent states in the accepting BSCC of $(\mathcal{M} \times \mathcal{A})_\pi$. Note that this policy has non-zero probability of being trapped in the accepting BSCC. Furthermore, note that $\sum_{s \in L^{-1}(home)} \text{Pr}^\infty_\pi (s) = \text{Pr}^\infty_\pi (s_0) = 0.76$, thereby satisfying the steady-state operator $\textbf{SS}_{[0.75, 1]} home$. In this example, the product LMC is a multichain; however, note that the original LMC over states $s \in S$ as given by the dashed component (ignoring the $q \in Q$ in each $(s, q) \in S^\times$) is a unichain. Furthermore, the two BSCCs of the multichain product LMC are identical with respect to their transition matrices due to the one-to-one correspondence of paths in the original LMC and the product LMC.


\section{Proof of Lemma~\ref{ordinarily-lumpable}}
\label{sec:ordinarily-lumpable}
By definition, the BSCC $(\hat{S}, \hat{T})$ is irreducible. We must show that, for all $s \in S$ and all $(s, q_\alpha), (s, q_\beta) \in [s]$, we have $(\mathbf{e}_\alpha - \mathbf{e}_\beta) \hat{T} V = 0$. Let $V \in \{0,
1\}^{(|S||Q|) \times |S|}$ such that $v_{(ij)k} = 1$ if $(s_i, q_j) \in
[s_k]$ and $v_{(ij)k} = 0$ otherwise. It follows that:
\begin{equation}
\begin{aligned}
    (\mathbf{e}_\alpha - \mathbf{e}_\beta) \hat{T} V = \left( \hat{T}(s, q_\alpha)(s_i, q_j) -  \hat{T}(s, q_\beta)(s_i, q_j) \right)_{\substack{i \leq |S| \\ j \leq |Q|}} V\\ 
    %(e_i - e_j) P V & = \left( T((s, q_1) | (s, q_i)) -  T((s, q_1) | (s, q_j)), \dots, T((s, q_m) | (s, q_i)) -  T((s, q_m) | (s, q_j)) \right) \\  
    = \left( \sum_{i \leq |S|, j \leq |Q|} v_{(ij)k} [\hat{T}(s, q_\alpha)(s_i, q_j) -  \hat{T}(s, q_\beta)(s_i, q_j)] \right)_{k \leq |S|}
    %& = \sum_{(s', q') \in S^\times} V((s', q'), [s_1]_R) [T((s', q') | (s, q_i)) -  T((s', q') | (s, q_j))], \dots, \sum_{(s', q') \in S^\times} V((s', q'), [s_n]_R) [T((s', q') | (s, q_i)) -  T((s', q') | (s, q_j))]
\end{aligned}
\end{equation}

\noindent Looking at the $k^\text{th}$ entry, we have:

\begin{equation}
    \sum_{(s_i, q_j) \in [s_k]} \hat{T}(s, q_\alpha)(s_i, q_j) -  \hat{T}(s, q_\beta)(s_i, q_j)
    \label{EntryK}
\end{equation}

%If $(s_i, q_j) \notin [s_k]_R$, then $v_{ijk} = 0$ and that term in the sum is
%0. If $v_{ijk} = 1$, T 

Two cases arise. First, let us consider the case where $[s] \neq [s_k]$. It follows from the definition of product LMCs that, for every transition from equivalence class $[s]$ to $[s_k]$, there are corresponding transitions $(s, q_\alpha)
\rightarrow (s_k, q_{\alpha'})$ and $(s, q_\beta) \rightarrow (s_k, q_{\beta'})$ (for some $\alpha', \beta'$) in $\Mm^\times$ such that $\hat{T}(s, q_\alpha)(s_k, q_{\alpha'}) = \hat{T}(s, q_\beta)(s_k,
q_{\beta'}) = T(s)(s_k)$. Thus, the sum equates to 0.
%  in this
% case. 
%Now, let us consider the case where $s = s_k$. Now, consider the case where
%$(s, q_\alpha), (s, q_\beta) \in [s_k]_R$. We have $v((s, q_i), [s]_R) = V((s,
%q_j), [s]_R) = 1$ and $V((s, q_i), [s']_R) = V((s, q_j), [s']_R) = 0$ for all
%$s' \neq s$.   

%Since $(s, q_i), (s, q_j) \in [s]_R$, it follows that, for any transition
%$[s]_R \rightarrow [s']_R$, we also have corresponding transitions $T((s',
%\cdot) | (s, q_i)) = T((s', \cdot) | (s, q_j)) = T(s' | s)$. Therefore, the
%preceding sum is equal to $0$ for all $[s_k]_R \neq [s]_R$.  

Now, assume $[s] = [s_k]$. Two cases arise. First, let us consider the case where
$[s]$ does not contain a self loop $T^\times (s, q)(s, q') > 0$ for some $q, q'$. Then all terms in the
preceding sum (\ref{EntryK}) are $T(s)(s) = 0$. Now, let us consider the case
where there is such a self loop so that $T(s)(s) > 0$. Then, since the DRA is
deterministic, there is exactly one successor $(s, q') \in [s]$ for any given
$(s, q) \in [s]$. From the pigeonhole principle, any trajectory of such product states resulting from the self loop must inevitably revisit some state, yielding a lollipop walk. For any two states, say $(s, q_i)$
and $(s, q_j)$, in this walk, there is exactly one successor yielding the term
$T(s)(s)$ for each of the two states. Thus, the sum in (\ref{EntryK}) equates
to 0. 

\noindent Since $s, \alpha, \beta$ were chosen arbitrarily, we have shown that $(\mathbf{e}_\alpha
- \mathbf{e}_\beta) \hat{T} V = 0$. 
% \end{proof}

\section{Proof of Theorem~\ref{theorem:aggregateLMC} and Corollary~\ref{corollary:aggregateIsOriginal}}
\label{sec:new-theorem}
% \begin{proof}
Given an irreducible LMC $\Mm = (S, \beta, T, R, AP, L)$ and some arbitrary DRA $\Aa$ with $m$ states, let the corresponding product LMC be given by $\Mm^\times = (S^\times, \beta^\times, T^\times,$ $ R^\times, AP, L^\times)$. Consider the partition $\bigcup_{s \in S} [s]$ given by the equivalence classes $[s] = \{ (s, q) | (s, q) \in S^\times \}$. We show that $\Mm = \Mm^*$, where $\Mm^* = (S^*, \beta^*, T^*, R^*,$ $ AP, L^*)$ denotes the aggregated LMC of $\Mm^\times$ under partition $\bigcup_{s \in S} [s]$. From Lemma 1, we know that this partition is ordinarily lumpable. Let $T([s])([s']) \in [0, 1]^{m \times m}$ denote the transition probability sub-matrix in $\Mm^\times$ shown below corresponding to transitions from states in $[s]$ to states in $[s']$. Per Theorem \ref{theorem:aggregateLMC}, we have that $T^*(s)(s') = \mathbf{e}_i T([s])([s']) \mathbf{e}^T$. Therefore, we must show that $T(s)(s') = \mathbf{e}_i T([s])([s']) \mathbf{e}^T$, where $i$ is an arbitrary index in $\{i | (s, q_i) \in S^\times \}$.

\begin{equation}
    T([s])([s']) = \left( \begin{matrix} T^\times (s, q_1)(s', q_1) & \cdots & T^\times (s, q_1)(s', q_m) \\ \vdots & \ddots & \vdots \\ T^\times (s, q_m)(s', q_1) & \cdots & T^\times (s, q_m)(s', q_m) \end{matrix} \right) 
\end{equation}
\noindent We have:
\begin{equation}
\begin{aligned}
    \nonumber
    T^*(s)(s') & = \mathbf{e}_i T([s])([s']) \mathbf{e}^T = \left( T^\times (s, q_i)(s', q_k) \right)_k \mathbf{e}^T \\ & = \sum_{k=1}^m T^\times (s, q_i)(s', q_k) = T^\times (s, q_i)(s', q') = T(s)(s')
\end{aligned}
\end{equation}

where $q' = \delta(q_i, L(s'))$ is the transition observed in the DRA. From Theorem \ref{theorem:aggregateLMC}, this establishes that the original LMC $\Mm$ and the aggregate LMC $\Mm^*$ have the same transition probability function $T = T^*$. The remaining equivalences follow from Definition \ref{def:quotient} and the definition of product LMCs. \qed
% \end{proof}

\section{Proof of Lemma~\ref{lemma:key}}
\label{sec:key-lemma}
The multichain transition probability matrix $T^\times$ is given by the canonical form in equation
(\ref{multichainT}) \cite{Puterman:1994}, where $W_k$ denotes transitions from transient states to the $k^\text{th}$ BSCC and $Z$ denotes transitions
between transient states.  
\begin{align}
    T^\times = \begin{bmatrix}
    T_1 & 0 & \ldots & 0  & 0 \\
    0 & T_2 & \dots & 0 & 0 \\
    \vdots & \vdots & \ddots & \vdots & \vdots \\
    0 & 0 & \ldots & T_m &  0 \\
    W_1 & W_2 & \ldots & W_m & Z
\end{bmatrix}
\label{multichainT}
\end{align}
    
%Without loss of generality, let us consider an irreducible Markov chain $M^* =
%(S^*, T^*)$, where $S^*$ contains exactly the states in the first BSCC and $T^*
%= T_1$.  
    
\noindent Recall the steady-state equations given below for the product LMC $\Mm^\times$.

\begin{equation}
\nonumber
\begin{aligned}
    (\text{Pr}^\infty (s_0, q_0), \dots) T^\times &= (\text{Pr}^\infty (s_0, q_0), \dots) \\ 
    \sum_{(s, q) \in S^\times} \text{Pr}^\infty (s, q) & = 1
\end{aligned}
\end{equation}
    
\noindent This yields the following system of linear equations for $\Mm^\times$:


\begin{equation}
\begin{aligned}
	& \text{Pr}^\infty (s, q) = \!\!\!\! \sum_{(s', q') \in S^k} \!\!\!\! \text{Pr}^\infty (s', q') T^\times (s', q')(s, q) \hspace*{12pt} \forall (s, q) \in S^k, k \\  
    & \sum_{k \leq m} \sum_{(s, q) \in S^k} \!\!\!\! \text{Pr}^\infty (s, q) = 1
\end{aligned}
\label{equation:isomorphicProof1}
\end{equation}
    
\noindent Similarly, we have the following equations for $\Mm'$:

\begin{equation}
\begin{aligned}
& \text{Pr}^\infty (s, q) = \sum_{(s', q') \in S'} \text{Pr}^\infty (s', q') T'(s', q')(s, q) \hspace*{12pt} \forall (s, q) \in S' \\ 
& \sum_{(s, q) \in S'} \!\!\!\! \text{Pr}^\infty (s, q) = 1
\end{aligned}
\label{equation:isomorphicProof2}
\end{equation}

    
Let $\langle s \rangle = \{(s, q) | (s, q) \text{ isomorphic in } T^G_1, \dots,
T^G_m \}$, where $T^G_k$ denotes the graph structure of $T_k$ in $M^\times$. See Figure \ref{fig:isomorphic} for an example. It follows from equations (\ref{equation:isomorphicProof1}) and (\ref{equation:isomorphicProof2}) that 
	
\begin{equation}
    \nonumber
    \begin{aligned}
    \sum_{(s, q) \in S'} \!\!\!\! & \text{Pr}^\infty (s, q) = \sum_{(s, q) \in S'} \sum_{(s', q') \in S'} T'(s', q')(s, q) \text{Pr}^\infty (s', q') = 1 \\ & = \sum_{k \leq m} \sum_{(s, q) \in S^k} \!\!\!\! \text{Pr}^\infty (s, q) = \sum_{k \leq m} \sum_{(s, q) \in S^k} \sum_{(s', q') \in S^k} \!\!\!\! T^\times (s', q')(s, q) \text{Pr}^\infty (s', q') \\ 
    & = \sum_{(s, q) \in S^1} \sum_{(s', q') \in S^1} T^\times (s', q')(s, q) \sum_{(s'', q'') \in \langle s' \rangle} \!\!\!\! \text{Pr}^\infty (s'', q'') \\ 
\end{aligned}
\end{equation}
    
The choice of $S^1$ in the last equation is arbitrary. Indeed, this result holds for any $S^k$. Therefore, $\text{Pr}^\infty (s, q) = \sum_{(s', q') \in \langle s \rangle} \text{Pr}^\infty (s', q')$ for all $(s, q) \in S'$.

\section{Proof of Lemma~\ref{lemma:key2}}
\label{sec:key2}
	%For any given state $s \in S$, two cases arise. First, $\mathcal{I}_s = 0$
	%implies that $\pi(a | s) = 0 = x_{sa}$ for all actions $a \in A(s)$. This
	%follows directly from constraints $(iii)$ and $(iv)$. The remainder of this
	%proof will focus on the case where $\mathcal{I}_s = 1$. Recall that
	%$\text{Pr}^\infty_\pi (s) = \sum_{a \in A(s)} x_{sa}$ is the steady-state
	%probability of $s$. Constraints $(i)$ and $(ii)$ are the well-known
	%steady-state probability equations.  
	
	Since $\pi(a | s, q) \in \{0, 1\}$ and we would like to prove that $x_{sqa} = \pi(a | s, q) \sum_a x_{sqa}$, we must show that $x_{sqa} \in \{0, \sum_a x_{sqa}\}$ such that $x_{sqa} = \sum_a x_{sqa}$ if and only if $\pi(a | s, q) = 1$. Note that $\sum_a x_{sqa} > 0$ because $(s, q)$ is recurrent. ($\implies$) The contrapositive statement $\pi(a | s, q) = 0$ implies $x_{sqa} = 0$ follows directly from constraint $(iii)$. ($\impliedby$) Since $\pi(a | s, q) = 1$, it follows from constraint $(iv)$ that $\sum_{a' \in A \setminus \{a\}} \pi (a' | s, q) = 0$. From constraint $(iii)$, we then have $\sum_{a' \in A \setminus \{a\}} x_{sqa'} = 0$. It follows that $x_{sqa} = \sum_a x_{sqa}$. 
	
	From the preceding arguments, we have $x_{sqa} = \pi(a | s, q) \text{Pr}^\infty_\pi (s, q)$. Since the product LMC has BSCCs with some shared state in $S$, it follows from Lemma 2 that the original LMC $\Mm_\pi$ will be a unichain. Thus, the solution to the steady-state equations (\ref{steadyStateEquations}) for $\Mm_\pi$ will be the unique stationary distribution reflecting the true steady-state behavior of the agent. We further have that this solution to equations (\ref{steadyStateEquations}) for $\Mm_\pi$ are obtained from $x$ in constraints $(i)$ and $(ii)$ per Lemma 3. Thus, $\pi(a | s, q) = x_{sqa} / \sum_a x_{sqa} \in \{0, 1\}$ is the policy which yields the steady-state distribution given by the solution to constraints $(i)$ through $(iv)$. 
	
	\section{Proof of Theorem~\ref{thm:main}}
    \label{sec:theorem-main}
	%Let $\mathcal{M}^\times = (S^\times, \beta^\times, A^\times, T^\times, R, Q, L^\times)$ denote the product LMDP resulting from $\mathcal{M}$ and the DRA $\mathcal{A} = \left( Q, q_0, \Sigma = 2^{AP}, \delta, \{(J_i, K_i)\}_{i \in [m]} \right)$ corresponding to $\phi_\text{LTL}$.
	%Let $S^k = \{s : \exists q, (s, q) \in S^\times\}$ denote the states in the BSCC of the product Markov chain induced by $\pi$ in the $k^\text{th}$ AMEC of the product MDP. We prove that $S^k = S^{k'}$ for all BSCCs in the product Markov chain. This implies that there is only one BSCC in the Markov chain induced by $\pi$ and that Markov chain is therefore irreducible. 
	($\implies$) We assume that $s_0$ is the initial state in the LMDP $\Mm$ (i.e. $\beta(s_0) = 1)$. Since the solution $(x, f, \pi, \mathcal{I})$ is feasible, there must be some $(s, q) \in S \times \bigcup_i G_i$ such that constraint $(xi)$ is satisfied. From constraint $(ix)$, note that this is only possible if $\mathcal{I}_{sq} = 1$, which is only possible if there is incoming flow into $(s, q)$ per the flow variables $f_{s'q'sq}$ in constraint $(vi)$. This corresponds to the outgoing flow of some neighboring state $(s', q')$. Again, from constraint $(vi)$, it follows that $(s', q')$ must also have incoming flow. By induction, we see that this holds for all states leading from the initial state $(s_0, \delta(q_0, L(s_0)))$ to $(s, q)$. Since positive flow is only enabled along edges  corresponding to actions chosen by the solution policy $\pi$ (per constraint $(v)$), it follows that there is a path from $(s_0, \delta(q_0, L(s_0)))$ to $(s, q)$ in the product LMC $(\Mm \times \Aa)_\pi$ and, due to the one-to-one correspondence between paths in the product LMC the original LMC $\Mm_\pi$, there is also a path from $s_0$ to $s$ in the latter. Now, consider the policy defined at state $(s, q)$. Since there is incoming flow, it follows from constraint $(viii)$ that there must also be outgoing flow. This flow will continue from state to state until some state is revisited, creating a BSCC. Constraints $(xii)$ through $(xvi)$ ensure that all such BSCCs contain the same states. In particular, note that the satisfaction of constraint $(xi)$ yields $\mathcal{I}^k = 1$ for the $k^\text{th}$ AMEC (without loss of generality) per constraint $(xii)$. Similarly, since $\mathcal{I}_{sq} = 1$, it follows from constraint $(xiv)$ that $\mathcal{I}^k_s = 1$ for that same AMEC. Constraint $(xiii)$ ensures that $\mathcal{I}^k_s$ cannot be set to $1$ unless there is some $\mathcal{I}_{sq} = 1$ in the $k^\text{th}$ AMEC. Thus, for any state $s \in S$ and $k$, we have $\mathcal{I}^k_s \leq \mathcal{I}^k$ and this is only met with equality if state $s \in S$ shows up in the BSCC corresponding to the $k^\text{th}$ AMEC. It follows that the sum $\sum_k (\mathcal{I}^k_s - \mathcal{I}^k)$ on the RHS of constraint $(xv)$ achieves its maximum value of $0$ if and only if state $s$ shows up in every BSCC of the product LMC $(\Mm \times \Aa)_\pi$. This must be the case per constraint $(xvi)$, which forces the LHS of constraint $(xv)$ to be $0$ for some state. From Lemma 2, this yields a unichain original LMC $\Mm_\pi$ in the original LMDP $\Mm$. From Theorem 1, Corollary 1, and Lemma 3, the satisfaction of constraints $(i)$, $(ii)$, and $(x)$ yields an LMC $\Mm_\pi$ satisfying the steady-state specifications in $\theta$. Finally, the satisfaction of constraints $(iii)$ and $(iv)$ ensure that the solution policy $\pi$ is deterministic.
	
	%Due to the one-to-one correspondence between paths in the original LMC and those in the product LMC, if some state $s \in S$ is visited in every BSCC of the latter, then it must be the case that $S^k = S^{k'}$ for all BSCCs in the product Markov chain.
		
	($\impliedby$) Assume we have a deterministic policy $\pi$ and the unichain original LMC induced by $\pi$ is given by $\mathcal{M}_\pi = (S, T_\pi)$ and satisfies the given SS+LTL specification $\theta$. We derive a feasible solution $(x, f, \pi, \mathcal{I})$ to program (\ref{equation:finalProgramss}). It follows from Lemma 2 that all BSCCs in the product LMC $(\mathcal{M} \times \Aa)_\pi$ obtained from $\Mm_\pi$ and the DRA $A$ of $\phi_\text{LTL}$ must contain the same states in $S$. 
	%That is, $S^k = S^{k'}$ for all BSCCs in the product LMC. 
	Let $\mathcal{I}_{sq} = \mathcal{I}_s = \mathcal{I}^k = \mathcal{I}^k_s = 1$ for all states $(s, q)$ in the BSCCs of $(\Mm \times \Aa)_\pi$ (these correspond to AMECs in the product LMDP $\Mm \times \Aa$). This satisfies constraints $(xii)$ through $(xvi)$. Note that the steady-state probabilities of such states must be positive and we can assign these values to $\sum_a x_{sqa}$ for every $(s, q)$ in the BSCCs. This satisfies $(i), (ii)$, and $(ix)$. Since the SS+LTL specification is satisfied, it must be the case that some state $(s, q) \in S \times \bigcup_i G_i$ is visited infinitely often, so we can assign the steady-state probability of such states to $\sum_a x_{sqa}$, thereby satisfying $(xi)$. Furthermore, since the steady-state operators in the specification are satisfied, it follows that constraint $(x)$ is satisfied. Note that constraints $(v)$ through $(viii)$ can be satisfied by setting the flow values to be proportional to the policy values. Finally, since $\pi(a | s, q) = x_{sqa} / \sum_a x_{sqa} \in \{0, 1\}$ ($\pi(a | s, q) = 0$) for recurrent (transient) states per Lemma 4, constraint $(iii)$ is satisfied and constraint $(iv)$ follows since deterministic policies are probability distributions.



==> ltlsynt.tex <==
% %Constraints $(i) - (xi)$ handle the steady-state operators \textbf{SS} of the
% %SSLTL controller synthesis problem.  
% We first focus on the linear-time portion given by operators \textbf{X, U}; that
% is, the LTL controller synthesis problem. The standard procedure is to compute a
% product LMDP between the underlying LMDP that models the agent-environment
% dynamics and the DRA that encodes the linear-time property. See Figure
% \ref{fig:example} for an example. Recall that a DRA $\mathcal{A}$ can be defined
% for any linear-time property $\phi$ such that the language of accepting traces
% in $\mathcal{A}$ corresponds to exactly the set of traces which satisfy $\phi$. 

% \begin{definition}[Product LMDP]
% 	\label{def:prodLMDP}
% 	Given an LMDP $\mathcal{M} = (S, \beta, A, T, R, AP, L)$ and a DRA
% 	$\mathcal{A} = \left( Q, q_0, \Sigma = 2^{AP}, \delta, \{(J_i, K_i)\}_{i \in
% 	[m]} \right)$, their product LMDP is given by $\mathcal{M}^\times =
% 	(S^\times, \beta^\times, A^\times, T^\times, R, Q, L^\times)$, where
% 	$S^\times = S \times Q$, the initial distribution $\beta^\times : S \times Q
% 	\mapsto [0, 1]$ is defined by $\beta(s, q) = \beta(s)$ if $q = \delta(q_0,
% 	L(s))$ and is $0$ otherwise, $T^\times : (S \times Q) \times A \times (S
% 	\times Q) \mapsto [0, 1]$ is defined in (\ref{eqn:TProd}), and $L^\times
% 	((s, q)) = \{q\}$. We denote by $A^\times((s, q)) = A(s)$ the actions
% 	available in state $(s, q) \in S^\times$. 
% \end{definition}

% \begin{equation}
% \begin{aligned}
% T^\times ((s', q') | (s, q), a) = 
% \begin{cases} 
% 	T(s' | s, a) & q' = \delta(q, L(s')) \\ 0 & \text{otherwise} 
% \end{cases}
% \end{aligned}
% \label{eqn:TProd}
% \end{equation}

% In the product LMDP, we are interested in finding end components (See
% Definitions \ref{def:MEC} and \ref{def:acceptingMEC}) which correspond to areas
% of the LMDP where $\phi$ may be satisfied by an appropriate policy where all the
% states in some such component are visited infinitely often. There is an
% algorithm which determines the maximal end components of a product LMDP in time
% $\mathcal{O}(|S^\times| (|S^\times| + |T^\times|))$
% \cite{principlesOfModelChecking}, where $|T^\times|$ is an abuse of notation
% denoting the number of transitions $((s, q), a, (s', q'))$ such that $T^\times
% ((s', q') | (s, q), a) > 0$. 

% \begin{figure}
% 	\includegraphics[width=\columnwidth]{example.PNG}
% 	\caption{(a) LMDP $\mathcal{M} = (S, \beta, A, T, R = \emptyset, AP, L)$,
% 	where $S = \{s_0, \dots, s_5\}$, $\beta(s_0) = 1$, $A = \{a_1, a_2, a_3\}$,
% 	$AP = \{a, b\}$, and $L(s_1) = L(s_2) = \{b\}, L(s_3) = L(s_4) = \{a\}$. The
% 	transition function is deterministic (i.e. $T: S \times A \times S \mapsto
% 	\{0, 1\}$) and shown in the figure by the transitions $a_i:1$ between states
% 	$s, s'$ denoting that $T(s' | s, a_i) = 1$. The blue transitions define a
% 	policy $\pi: S \times A \mapsto \{0, 1\}$ which induces an LMC
% 	$\mathcal{M}_\pi$. (b) Given the LTL specification $(\textbf{F } a)
% 	\textbf{ U } b$, the LTL DRA $\mathcal{A} = (Q, q_0, \Sigma, \delta, F =
% 	\{(J_i, K_i)\}_i)$ is defined, where $Q = \{q_0, q_1, q_2, q_3\}$, $\Sigma =
% 	2^{AP}$, $F = \{(\emptyset, \{q_2\})\}$, and the transition function is
% 	given by $\delta(q_0, \{a\}) = q_0, \delta(q_0, \emptyset) = q_1,
% 	\delta(q_0, \{b\}) = q_2, \delta(q_1, \{a\}) = q_0, \delta(q_1, \emptyset) =
% 	q_1, \delta(q_1, \{b\}) = q_3, \delta(q_3, \{a\}) = q_2, \delta(q_3, \{b\}),
% 	\delta(q_3, \{a\}) = q_2, \delta(q_2, \cdot) = q_2$. (c) Product LMDP
% 	$\mathcal{M} \times \mathcal{A}$, where red nodes represent states in the
% 	accepting MEC of $\mathcal{M} \times \mathcal{A}$. The blue transitions
% 	define the LMC $(\mathcal{M} \times \mathcal{A})_\pi$ induced by the policy
% 	$\pi$ given by the blue transitions in (a) for the LMDP $\mathcal{M}$. Note
% 	that this policy induces an LMC that has probability 1 of being trapped in
% 	the accepting MEC. Therefore, the probability of satisfying $(\textbf{F } a)
% 	\textbf{ U } b$ given that we start in state $s_0$ is 1.} 
% 	\label{fig:example}
% \end{figure}


% \begin{definition}[Maximal End Component]
% 	Given the product LMDP $\mathcal{M}^\times = (S^\times, \beta^\times,
% 	A^\times, $ $T^\times, Q, L^\times)$ of an LMDP $\mathcal{M} = (S, \beta, A,
% 	T, AP, L)$ and a DRA $\mathcal{A} = \left( Q, q_0, \Sigma = 2^{AP}, \delta,
% 	\right.$ $\left. \{(J_i, K_i)\}_{i \in [m]} \right)$, an end component $E =
% 	(S^E, A^E), S^E \subseteq S^\times, A^E (s) \subseteq A^\times (s)$ is a
% 	sub-MDP of $\mathcal{M}$ such that the digraph formed by $E$ is strongly
% 	connected. An end component is said to be maximal if it is not contained in
% 	any other end component.  
% 	\label{def:MEC}
% \end{definition}

% %\begin{definition}[Maximal End Component]
% %   Given an LMDP $\mathcal{M} = (S, \beta, A, T, R, \Sigma, L)$, an end
% %   component $E = (S^E, A^E), S^E \subseteq S, A^E (s) \subseteq A(s)$ is a
% %   sub-MDP of $\mathcal{M}$ such that the digraph formed by $E$ is strongly
% %   connected. An end component is said to be maximal if it is not contained in
% %   any other end component.  
% %	\label{def:MEC}
% %\end{definition}

% %For all end components $E = (S^E, A^E)$, there exists a policy which will visit
% %every state $s \in S^E$ infinitely often. It is also the case that, for any
% %MDP, all policies will induce a Markov chain whose probability of reaching some
% %end component is $1$ \cite{ECProb}. 


% \begin{definition}[Accepting Maximal End Component \cite{principlesOfModelChecking}]
% 	%Given the product LMDP $\mathcal{M}^\times = (S^\times, \beta^\times,
% 	%A^\times, T^\times, Q, L^\times)$ of an LMDP $\mathcal{M} = (S, \beta, A,
% 	%T, \Sigma, L)$ and a DRA $\mathcal{A} = \left( Q, q_0, 2^\Sigma, \delta,
% 	%\{(J_i, K_i)\}_{i \in [m]} \right)$,  
% 	An accepting maximal end component $E = (S^E, A^E)$ is a maximal end
% 	component of $\mathcal{M}^\times$ such that $S^E \cap (S \times J_i) =
% 	\emptyset$ and $S^E \cap (S \times K_i) \neq \emptyset$ for some $i \in
% 	[m]$. 
% 	%\textcolor{blue}{(updated acceptance conditions based on \cite[pg.
% 	%803]{principlesOfModelChecking})} 
% 	\label{def:acceptingMEC}
% \end{definition}

As with LMDPs and LMCs, any solution policy $\pi$ induces a product LMC in the
underlying product LMDP. These LMCs have analogues to the maximal end components
of LMDPs, known in this case as accepting bottom strongly connected components.
See Figure \ref{fig:example2} for an example. 

\begin{definition}[Product LMC]
	Given an LMC $\mathcal{M} = (S, \beta, T, AP, L)$ and a DRA $\mathcal{A} =
	(Q, q_0, \Sigma = 2^{AP}, \delta, {(J_i, K_i)}_{i \in [m]})$, the product
	Markov chain is given by $\mathcal{M} \times \mathcal{A} = (S^\times,
	\beta^\times, T^\times, $ $Q, L^\times)$, where $L^\times ((s, q)) = \{q\}$
	and $\beta^\times, T^\times$ are given by: 
	%\{\text{accept}\}$ if $q \in  %. $L' : S \times Q \mapsto 2^{F'}, F' =
	%\{J_1, \dots, J_m, K_1, \dots, K_m\} \text{ such that } H \in L'((s, q))
	%\text{ iff } q \in H$.   
	\begin{gather}
	\nonumber
	\begin{aligned}
	\beta^\times ((s, q)) = 
	\begin{cases} 
		\beta (s) & q = \delta(q_0, L(s)) \\ 0 & \text{otherwise} 
	\end{cases} \\ 
	T^\times ((s', q') | (s, q)) = 
	\begin{cases} 
		T(s' | s) & q' = \delta(q, L(s')) \\ 0 & \text{otherwise} 
	\end{cases} \\ 
	% = \begin{cases} \text{accept} & q \in F \\ \emptyset & \text{otherwise} \end{cases} 
	\end{aligned}
	\end{gather}
	\label{def:prodLMC}
\end{definition}

\begin{definition}[Bottom Strongly Connected Component]
	Given an LMC $\mathcal{M} = (S, \beta, T, AP, $ $L)$, a Bottom Strongly
	Connected Component (BSCC) is a closed strongly connected component $S^B
	\subseteq S$. That is, one which, when entered, is never left. 
	\label{def:BSCC}
\end{definition}

\begin{definition}[Accepting BSCC]
	Given a product LMC $\mathcal{M} \times \mathcal{A} = (S^\times,
	\beta^\times, T^\times, Q, L^\times)$ of LMC $\mathcal{M} = (S, \beta, T,
	AP, L)$ and DRA $\mathcal{A} = (Q, q_0, \Sigma = 2^{AP}, \delta, \{J_i,
	K_i\}_{i \in [m]})$, an accepting BSCC $S^B \subseteq S^\times$ of
	$\mathcal{M} \times \mathcal{A}$ is a BSCC such that, for some $i \in [m]$,
	we have $S^B \cap (S \times J_i) = \emptyset$ and $S^B \cap (S \times K_i)
	\neq \emptyset$. 
	\label{def:acceptingBSCC}
\end{definition}

There is a one-to-one correspondence between the probability of an LMC
$\mathcal{M}$ satisfying a given LTL specification $\phi$ and the probability of
reaching some accepting BSCC in the product LMC $\mathcal{M} \times
\mathcal{A}$, where $\mathcal{A}$ is the DRA corresponding to $\phi$.   

Given an LMDP $\mathcal{M} = (S, \beta, A, T, R, \Sigma, L)$, the maximum
probability of a state $s$ satisfying a given linear-time property $\phi$ can be
reduced to the problem of determining the maximum probability of reaching an
accepting MEC in the product MDP $\mathcal{M}^\times$ of $\mathcal{M}$ and the
DRA corresponding to $\phi$. Indeed, it has been shown that, given an arbitrary
LTL formula $\phi$ and LMDP $\mathcal{M}$, the policy which maximizes the
probability of reaching an accepting MEC in $\mathcal{M}^\times$ also yields a
policy which maximizes the probability of satisfying $\phi$ in $\mathcal{M}$
\cite{maxProbs}. Once an accepting MEC is reached, one must simply choose
actions in the MEC infinitely often in order to ensure that all states within it
are visited infinitely often. It is worth noting that the policy $\pi: S \times
A \rightarrow \{0, 1\}$ which maximizes the probability of satisfying $\phi$ for
the original LMDP $\mathcal{M}$ can be trivially determined from $\pi^\times$ as
it has been shown that $\pi(a | s) = \pi^\times (a | (s, q)), s \in S, q \in Q$
~\cite{CITE}.  

There is a crucial distinction to be made at this point. Whereas traditional LTL
controller synthesis is agnostic to the actions taken when the agent reaches an
AMEC, the addition of steady-state specifications makes such choice of actions
critical as these can clearly affect the resulting steady-state probabilities of
the Markov chain induced by the solution policy. For the remainder of this
paper, we focus on the derivation of optimal policies which satisfy a logic
fragment of SSTL, which we call SSTL$_\perp$, wherein the steady-state operator
\textbf{SS} cannot be nested within path operators. That is, an SSTL$_\perp$
formula takes the form of $\theta = \phi_\text{LTL} \wedge \bigwedge_i
\textbf{SS}_{l_i, u_i} p_i$. 

\begin{figure}[ht!]
	\includegraphics[width=\columnwidth]{example2.PNG}
	\caption{(a) LMDP $\mathcal{M} = (S, \beta, A, T, R = \emptyset, AP, L)$,
	where $S = \{s_0, \dots, s_8\}$, $\beta(s_0) = 1$, $A = \{\leftarrow,
	\downarrow, \rightarrow, \uparrow\}$, $AP = \{home, danger, tool\}$, and
	$L(s_0) = \{home\}, L(s_1) = L(s_7) = \{danger\}, L(s_8) = \{tool\}$. the
	agent has a chance of slipping whenever it moves, causing a transition into
	one of three possible states. If the agent chooses to go right (left), there
	is an 80$\%$ chance that it will transition to the right (left), and the
	chance of transitioning to either of the states above or below it is 10$\%$.
	Similarly, if the agent chooses to up (down), it will end up in the states
	above (below) it with 80$\%$ chance, and in the states to the right and left
	of it with chance 10$\%$ each. In the corners of the map, the agent may stay
	in place with 90$\%$ probability by choosing to move against the boundary of
	the map (e.g. $T(s_0 | s_0, \leftarrow) = 0.9$). (b) Given the SSTL
	specification $(! danger \textbf{U} tool) \wedge \textbf{SS}_{[0.75, 1]}
	home$, the LTL DRA $\mathcal{A} = (Q, q_0, \Sigma, \delta, F = \{(J_i,
	K_i)\}_i)$ is defined, where $Q = \{q_0, q_1, q_2\}$, $\Sigma = 2^{AP}$, $F
	= \{(\emptyset, \{q_1\})\}$, and the transition function is given by
	$\delta(q_0, \{home\}) = q_0, \delta(q_0, \{tool\}) = q_1, \delta(q_0,
	\{danger\}) = q_2, \delta(q_1, \cdot) = q_1, \delta(q_2, \cdot) = q_2$. The
	steady-state operator is not used in defining $\mathcal{A}$. (c) Product LMC
	$(\mathcal{M} \times \mathcal{A})_\pi$ induced by the policy $\pi$ given by
	the black arrows in (a) for the product LMDP $\mathcal{M} \times
	\mathcal{A}$, where red nodes represent states in the accepting BSCC of
	$(\mathcal{M} \times \mathcal{A})_\pi$. Note that this policy has non-zero
	probability of being trapped in the accepting BSCC. Furthermore, note that
	$\sum_{s \in \mathcal{L}_{home}} \text{Pr}^\infty_\pi (s) =
	\text{Pr}^\infty_\pi (s_0) = 0.76$, thereby satisfying the steady-state
	specification $\textbf{SS}_{[0.75, 1]} home$.} 
	\label{fig:example2}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% TeX-PDF-mode: t
%%% End:
